Observation of the $B^0\rightarrow\overline{D}^{*0}K^{+}\pi^{-}$ and $B_s^0\rightarrow\overline{D}^{*0}K^{-}\pi^{+}$ decays

The first observations of $B^0\rightarrow\overline{D}^{*}(2007)^{0}K^{+}\pi^{-}$ and $B_s^0\rightarrow\overline{D}^{*}(2007)^{0}K^{-}\pi^{+}$ decays are presented, and their branching fractions relative to that of the $B^0\rightarrow\overline{D}^{*}(2007)^{0}\pi^{+}\pi^{-}$ decay are reported. These modes can potentially be used to investigate the spectroscopy of charm and charm-strange resonances and to determine the angle $\gamma$ of the CKM unitarity triangle. It is also important to understand them as a source of potential background in determinations of $\gamma$ from $B^{+}\rightarrow DK^{+}$ and $B^{0}\rightarrow DK^{+}\pi^{-}$ decays. The analysis is based on a sample corresponding to an integrated luminosity of $5.4 ~\rm{fb}^{-1}$ of proton--proton collision data at $13 ~\rm{TeV}$ centre-of-mass energy recorded with the LHCb detector. The $\overline{D}^{*}(2007)^{0}$ mesons are fully reconstructed in the $\overline{D}^{0}\pi^{0}$ and $\overline{D}^{0}\gamma$ channels, with the $\overline{D}^{0} \rightarrow K^{+}\pi^{-}$ decay. A novel weighting method is used to subtract background while simultaneously applying an event-by-event efficiency correction to account for resonant structures in the decays.

==> Authorship_LHCb-PAPER-2021-043-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abell{\'a}n Beteta,
F. Abudin{\'e}n,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C. Agapopoulou,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista de Souza Leite,
M. Barbetti,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
A. Bertolin,
C. Betancourt,
F. Betti,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
N.V. Biesuz,
S. Bifani,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
P. Campana,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
D. Cervenkov,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
I. Corredoira ,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Dashkina,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
F. De Vellis,
J.A. de Vries,
C.T. Dean,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Cicco,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
L.N. Falcao,
Y. Fan,
B. Fang,
S. Farry,
D. Fazzini,
M. F{\'e}o,
A. Fernandez Prieto,
A.D. Fernez,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
A. Fkiaras,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
E. Gabriel,
G. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
L. Giambastiani,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
M. Guittiere,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
S.C. Haines,
T. Halewood-leagas,
P.M. Hamilton,
J.P. Hammerich,
Q. Han,
X. Han,
E.B. Hansen,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
R. Hou,
Y. Hou,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
X. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
D. Karpenkov,
M. Karpov,
J.W. Kautz,
F. Keizer,
D.M. Keller,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
J. Kubat,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
P. Li,
S. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
Q. Liu,
S. Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
S. L{\'o}pez Soli{\~n}o,
G.H. Lovell,
Y. Lu,
C. Lucarelli,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
J. Marks,
A.M. Marshall,
P.J. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
N.T. Mchugh,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
G. Meier,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
A. Minotti,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
R. Murta,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Normand,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
D.P. O'Hanlon,
S. Okamura,
R. Oldeman,
F. Oliva,
M.E. Olivares,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
O. Ozcelik,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
A. Pereiro Castro,
P. Perret,
M. Petric,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
R. Piandani,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
M. Pizzichemi,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
V. Puill,
G. Punzi,
H. Qi,
W. Qian,
N. Qin,
R. Quagliani,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
A.M. Ricci,
S. Ricciardi,
K. Rinnert,
P. Robbe,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
E.R.R. Rodriguez Rodriguez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
E.B. Shields,
Y. Shimizu,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
R. Skuza,
T. Skwarnicki,
M.W. Slater,
I. Slazyk,
J.C. Smallwood,
J.G. Smeaton,
E. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
S. Stone,
D. Strekalina,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
A.R. Tanner,
M.D. Tat,
A. Terentev,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
K.A. Thomson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
X. Tong,
D. Torres Machado,
D.Y. Tou,
E. Trifonova,
S.M. Trilov,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
M. Van Dijk,
H. Van Hecke,
E. van Herwijnen,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
K. Vos,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
N.K. Watson,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M. K. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
S. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zharkova,
A. Zhelezov,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
X. Zhu,
X. Zhu,
Z. Zhu,
V. Zhukov,
Q. Zou,
S. Zucchelli,
D. Zuliani,
G. Zunica
